Compressing Pre-trained Transformers via Low-Bit NxM Sparsity for Natural Language Understanding

In recent years, large pre-trained Transformer networks have demonstrated dramatic improvements in many natural language understanding tasks. However, the huge size of these models brings significant challenges to their fine-tuning and online deployment due to latency and cost constraints. New hardware supporting both N:M semi-structured sparsity and low-precision integer computation is a promising solution to boost DNN model serving efficiency. However, there have been very few studies that systematically investigate to what extent pre-trained Transformer networks benefit from the combination of these techniques, as well as how to best compress each component of the Transformer. We propose a flexible compression framework NxMiFormer that performs simultaneous sparsification and quantization using ADMM and STE-based QAT. Furthermore, we present and inexpensive, heuristic-driven search algorithm that identifies promising heterogeneous compression configurations that meet a compression ratio constraint. When evaluated across the GLUE suite of NLU benchmarks, our approach can achieve up to 93% compression of the encoders of a BERT model while retaining 98.2% of the original model accuracy and taking full advantage of the hardware's capabilities. Heterogeneous configurations found the by the search heuristic maintain 99.5% of the baseline accuracy while still compressing the model by 87.5%.

==> spacing.tex <==
\usepackage[skip=2pt]{caption}
\usepackage{setspace}
\usepackage{enumitem}
\usepackage{titlesec}

% \captionsetup[subfloat]{captionskip=1pt}
% \captionsetup[subfloat]{captionskip=1pt}

% % \newtoggle{tech-report}
% % \toggletrue{tech-report}
% % % \togglefalse{tech-report}

% % \iftoggle{tech-report}{%
% % }{
% \renewcommand{\baselinestretch}{1}
% % }

\setlist{nosep} % Change space between items in a listing.
\setlength{\textfloatsep}{2pt} % Control space after figure and before text. 
\setlength{\dbltextfloatsep}{2pt}

% \setlength{\intextsep}{2ex} % remove extra space above and below in-line float (reduce space in between figure caption and the text below it)

% \newlength{\sectionbelowskip}
% \newlength{\sectionaboveskip}
% \newlength{\subsectionbelowskip}
% \newlength{\subsectionaboveskip}
% \newlength{\subsubsectionbelowskip}
% \newlength{\subsubsectionaboveskip}
% \newlength{\paragraphaboveskip}
% \newlength{\paragraphbelowskip}

%  Control space before and after table
% \newcommand{\spaceabovetable}{\vspace*{-1em}}
% \newcommand{\spacebelowtable}{\vspace*{-1em}}
% \newcommand{\spaceabovetable}{\vspace*{2em}}
% \newcommand{\spacebelowtable}{\vspace*{2em}}

% \usepackage{titlesec-custom}

% % Avoid starting a new line for subsubsection
% % \makeatletter
% % \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
% %                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
% %                                      {-1.5ex \@plus -.2ex}% Formerly 1.5ex \@plus .2ex
% %                                      {\normalfont\normalsize\bfseries}}
% % \makeatother

% \titleformat{\subsubsection}[runin]% runin puts it in the same paragraph
%         {\normalfont\normalsize\bfseries}% formatting commands to apply to the whole heading
%         {\thesubsubsection}% the label and number
%         {0.5em}% space between label/number and subsection title
%         {}% formatting commands applied just to subsection title
%         [.]% punctuation or other commands following subsection title
% \titleformat{\subsubsection}
%   {\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}
% \titlespacing*{\subsubsection}{0pt}{\subsubsectionaboveskip}{\subsubsectionbelowskip}

% \newcommand{\setvspace}[2]{%
%   #1 = #2
%   \advance #1 by -1\parskip}

% Ever so slightly tighter than defaults:
% \setvspace{\sectionaboveskip}{4pt plus 1pt minus 1pt}
% \setlength{\sectionbelowskip}{2pt plus 1pt minus 1pt}
% \setlength{\subsectionbelowskip}{2pt plus 2pt minus 0pt}
% \setvspace{\subsectionaboveskip}{1pt plus 2pt minus 2pt}
% % \setlength{\subsubsectionbelowskip}{1pt plus 0pt minus 2pt}
% % \setvspace{\subsubsectionaboveskip}{1pt plus 0pt minus 2pt}
% \setvspace{\paragraphaboveskip}{1pt}
% \setvspace{\paragraphbelowskip}{1pt}
% \setvspace{\sectionaboveskip}{1pt plus 4pt minus 2pt}
% \setlength{\sectionbelowskip}{1pt plus 2pt minus 2pt}
% \setvspace{\subsectionaboveskip}{1pt plus 2pt minus 2pt}
% \setlength{\subsectionbelowskip}{0pt plus 2pt minus 2pt}
% \setvspace{\subsubsectionaboveskip}{1pt plus 4pt minus 2pt}
% \setlength{\subsubsectionbelowskip}{1pt plus 4pt minus 2pt}
% \setvspace{\paragraphaboveskip}{1pt}
% \setvspace{\paragraphbelowskip}{1pt}


% % \titlespacing*{\section}{0pt}{\sectionaboveskip}{\sectionbelowskip}
% \titlespacing{\subsection}{0pt}{0pt}{0pt}
% \titlespacing*{\paragraph}{1pt}{\paragraphaboveskip}{*}


\makeatletter % Control space around theorem and lemma
\def\thm@space@setup{%
  \thm@preskip=3pt
  \thm@postskip=\thm@preskip % or whatever, if you don't want them to be equal
}
\makeatother

% % Control space around itemize items
\setlist[itemize]{noitemsep, topsep=0pt}

% control space above and below equation.
\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

\makeatletter % Control the space around the proof.
\renewenvironment{proof}[1][\proofname]{\par
  \vspace{1pt}% remove the space after the theorem
  \pushQED{\qed}%
  \normalfont
  \topsep0pt \partopsep0pt % no space before
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
  \addvspace{3pt plus 3pt} % some space after
}
\makeatother 

% \setlength{\itemindent}{0em}
